Context-Sensitive Abstract Interpretation of Dynamic Languages

There is a vast gap in the quality of IDE tooling between static languages like Java and dynamic languages like Python or JavaScript. Modern frameworks and libraries in these languages heavily use their dynamic capabilities to achieve the best ergonomics and readability. This has a side effect of making the current generation of IDEs blind to control flow and data flow, which often breaks navigation, autocompletion and refactoring. In this thesis we propose an algorithm that can bridge this gap between tooling for dynamic and static languages by statically analyzing dynamic metaprogramming and runtime reflection in programs. We use a technique called abstract interpretation to partially execute programs and extract information that is usually only available at runtime. Our algorithm has been implemented in a prototype analyzer that can analyze programs written in a subset of JavaScript.

==> background.tex <==
\chapter{Background}

\section{Sensitivity in static analysis}

A static analysis is sensitive to a given aspect of program execution if it can distinguish
between data flows that differ in this aspect, but otherwise would look the same.

\subsubsection{Context-sensitive analysis}

Analysis is context-sensitive if it is able to distinguish between different calls to
the same function. For example, ...

\subsubsection{Flow-sensitive analysis}

Analysis is flow-sensitive if it understands that mutable memory can be overwritten
and that reading from it can only see the most recently written value.

\subsubsection{Loop-sensitive analysis}

Analysis is loop-sensitive if it can distinguish between data that is read or written
during different iterations of a loop.

\subsubsection{Allocation-sensitive analysis}

Analysis is allocation-sensitive if it can distinguish between different objects that
have been allocated at the place in the program.

\section{Abstract interpretation as a framework for building program analyzers}

TODO


==> discussion.tex <==

\chapter{Discussion and Outlook}
  \label{Discussion}

Of course very important! You need to discuss the informatics as well as bio part of your thesis topic.

\bigskip
Take your time for writing the discussion, besides the introduction chapter it is the most important chapter of your thesis.
Also do not subsection the discussion too heavily.
\clearpage
At least 5 pages.
\clearpage
Outlook can become an extra chapter.

